On Taking Advantage of Opportunistic Meta-knowledge to Reduce Configuration Spaces for Automated Machine Learning

The automated machine learning (AutoML) process can require searching through complex configuration spaces of not only machine learning (ML) components and their hyperparameters but also ways of composing them together, i.e. forming ML pipelines. Optimisation efficiency and the model accuracy attainable for a fixed time budget suffer if this pipeline configuration space is excessively large. A key research question is whether it is both possible and practical to preemptively avoid costly evaluations of poorly performing ML pipelines by leveraging their historical performance for various ML tasks, i.e. meta-knowledge. The previous experience comes in the form of classifier/regressor accuracy rankings derived from either (1) a substantial but non-exhaustive number of pipeline evaluations made during historical AutoML runs, i.e. 'opportunistic' meta-knowledge, or (2) comprehensive cross-validated evaluations of classifiers/regressors with default hyperparameters, i.e. 'systematic' meta-knowledge. Numerous experiments with the AutoWeka4MCPS package suggest that (1) opportunistic/systematic meta-knowledge can improve ML outcomes, typically in line with how relevant that meta-knowledge is, and (2) configuration-space culling is optimal when it is neither too conservative nor too radical. However, the utility and impact of meta-knowledge depend critically on numerous facets of its generation and exploitation, warranting extensive analysis; these are often overlooked/underappreciated within AutoML and meta-learning literature. In particular, we observe strong sensitivity to the `challenge' of a dataset, i.e. whether specificity in choosing a predictor leads to significantly better performance. Ultimately, identifying `difficult' datasets, thus defined, is crucial to both generating informative meta-knowledge bases and understanding optimal search-space reduction strategies.

==> sections/automl_predictor_heatmap.tex <==

\begin{figure}[!htbp]  
  \centering 
  \subfloat[abalone]{
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_abalone_color_flatten.pdf}
      }
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using prior evaluations of AutoML. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_automl_predictor_per_dataset}
\end{figure}
 
\begin{figure}[!htbp] 
\ContinuedFloat 
  \centering 
    \subfloat[adult]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_adult_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using prior evaluations of AutoML. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_automl_predictor_per_dataset}
\end{figure}

\begin{figure}[!htbp] 
\ContinuedFloat 
  \centering 
    \subfloat[amazon]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_amazon_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using prior evaluations of AutoML. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_automl_predictor_per_dataset}
\end{figure}


\begin{figure}[!htbp] 
\ContinuedFloat 
  \centering 
    \subfloat[car]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_car_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using prior evaluations of AutoML. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_automl_predictor_per_dataset}
\end{figure}


\begin{figure}[!htbp] 
\ContinuedFloat 
  \centering 
    \subfloat[cifar10small]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_cifar10small_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using prior evaluations of AutoML. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_automl_predictor_per_dataset}
\end{figure}


\begin{figure}[!htbp] 
\ContinuedFloat 
  \centering 
    \subfloat[convex]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_convex_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using prior evaluations of AutoML. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_automl_predictor_per_dataset}
\end{figure}


\begin{figure}[!htbp] 
\ContinuedFloat 
  \centering 
    \subfloat[dexter]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_dexter_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using prior evaluations of AutoML. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_automl_predictor_per_dataset}
\end{figure}


\begin{figure}[!htbp] 
\ContinuedFloat 
  \centering 
    \subfloat[dorothea]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_dorothea_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using prior evaluations of AutoML. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_automl_predictor_per_dataset}
\end{figure}


\begin{figure}[!htbp] 
\ContinuedFloat 
  \centering 
    \subfloat[gcredit]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_gcredit_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using prior evaluations of AutoML. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_automl_predictor_per_dataset}
\end{figure}


\begin{figure}[!htbp] 
\ContinuedFloat 
  \centering 
    \subfloat[gisette]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_gisette_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using prior evaluations of AutoML. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_automl_predictor_per_dataset}
\end{figure}


\begin{figure}[!htbp] 
\ContinuedFloat 
  \centering 
    \subfloat[kddcup]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_kddcup_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using prior evaluations of AutoML. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_automl_predictor_per_dataset}
\end{figure}


\begin{figure}[!htbp] 
\ContinuedFloat 
  \centering 
    \subfloat[krvskp]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_krvskp_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using prior evaluations of AutoML. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_automl_predictor_per_dataset}
\end{figure}


\begin{figure}[!htbp] 
\ContinuedFloat 
  \centering 
    \subfloat[madelon]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_madelon_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using prior evaluations of AutoML. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_automl_predictor_per_dataset}
\end{figure}


\begin{figure}[!htbp] 
\ContinuedFloat 
  \centering 
    \subfloat[mnist]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_mnist_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using prior evaluations of AutoML. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_automl_predictor_per_dataset}
\end{figure}


\begin{figure}[!htbp] 
\ContinuedFloat 
  \centering 
    \subfloat[secom]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_secom_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using prior evaluations of AutoML. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_automl_predictor_per_dataset}
\end{figure}


\begin{figure}[!htbp] 
\ContinuedFloat 
  \centering 
    \subfloat[semeion]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_semeion_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using prior evaluations of AutoML. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_automl_predictor_per_dataset}
\end{figure}


\begin{figure}[!htbp] 
\ContinuedFloat 
  \centering 
    \subfloat[shuttle]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_shuttle_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using prior evaluations of AutoML. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_automl_predictor_per_dataset}
\end{figure}


\begin{figure}[!htbp] 
\ContinuedFloat 
  \centering 
    \subfloat[waveform]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_waveform_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using prior evaluations of AutoML. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_automl_predictor_per_dataset}
\end{figure}


\begin{figure}[!htbp] 
\ContinuedFloat 
  \centering 
    \subfloat[winequality]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_winequality_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using prior evaluations of AutoML. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_automl_predictor_per_dataset}
\end{figure}


\begin{figure}[!htbp] 
\ContinuedFloat 
  \centering 
    \subfloat[yeast]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_yeast_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using prior evaluations of AutoML. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_automl_predictor_per_dataset}
\end{figure}
 

==> sections/default_predictor_heatmap.tex <==


\begin{figure}[h] 
  \centering 
    \subfloat[abalone]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_abalone_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using 10 fold-cv evaluations with default hyperparameters. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_default_predictor_per_dataset}
\end{figure}
 
\begin{figure}[h]
\ContinuedFloat 
  \centering 
    \subfloat[adult]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_adult_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using 10 fold-cv evaluations with default hyperparameters. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_default_predictor_per_dataset}
\end{figure}

\begin{figure}[h]
\ContinuedFloat 
  \centering 
    \subfloat[amazon]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_amazon_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using 10 fold-cv evaluations with default hyperparameters. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_default_predictor_per_dataset}
\end{figure}


\begin{figure}[h]
\ContinuedFloat 
  \centering 
    \subfloat[car]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_car_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using 10 fold-cv evaluations with default hyperparameters. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_default_predictor_per_dataset}
\end{figure}


\begin{figure}[h]
\ContinuedFloat 
  \centering 
    \subfloat[cifar10small]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_cifar10small_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using 10 fold-cv evaluations with default hyperparameters. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_default_predictor_per_dataset}
\end{figure}


\begin{figure}[h]
\ContinuedFloat 
  \centering 
    \subfloat[convex]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_convex_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using 10 fold-cv evaluations with default hyperparameters. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_default_predictor_per_dataset}
\end{figure}


\begin{figure}[h]
\ContinuedFloat 
  \centering 
    \subfloat[dexter]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_dexter_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using 10 fold-cv evaluations with default hyperparameters. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_default_predictor_per_dataset}
\end{figure}


\begin{figure}[h]
\ContinuedFloat 
  \centering 
    \subfloat[dorothea]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_dorothea_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using 10 fold-cv evaluations with default hyperparameters. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_default_predictor_per_dataset}
\end{figure}


\begin{figure}[h]
\ContinuedFloat 
  \centering 
    \subfloat[gcredit]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_gcredit_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using 10 fold-cv evaluations with default hyperparameters. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_default_predictor_per_dataset}
\end{figure}


\begin{figure}[h]
\ContinuedFloat 
  \centering 
    \subfloat[gisette]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_gisette_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using 10 fold-cv evaluations with default hyperparameters. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_default_predictor_per_dataset}
\end{figure}


\begin{figure}[h]
\ContinuedFloat 
  \centering 
    \subfloat[kddcup]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_kddcup_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using 10 fold-cv evaluations with default hyperparameters. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_default_predictor_per_dataset}
\end{figure}


\begin{figure}[h]
\ContinuedFloat 
  \centering 
    \subfloat[krvskp]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_krvskp_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using 10 fold-cv evaluations with default hyperparameters. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_default_predictor_per_dataset}
\end{figure}


\begin{figure}[h]
\ContinuedFloat 
  \centering 
    \subfloat[madelon]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_madelon_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using 10 fold-cv evaluations with default hyperparameters. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_default_predictor_per_dataset}
\end{figure}


\begin{figure}[h]
\ContinuedFloat 
  \centering 
    \subfloat[mnist]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_mnist_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using 10 fold-cv evaluations with default hyperparameters. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_default_predictor_per_dataset}
\end{figure}


\begin{figure}[h]
\ContinuedFloat 
  \centering 
    \subfloat[secom]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_secom_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using 10 fold-cv evaluations with default hyperparameters. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_default_predictor_per_dataset}
\end{figure}


\begin{figure}[h]
\ContinuedFloat 
  \centering 
    \subfloat[semeion]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_semeion_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using 10 fold-cv evaluations with default hyperparameters. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_default_predictor_per_dataset}
\end{figure}


\begin{figure}[h]
\ContinuedFloat 
  \centering 
    \subfloat[shuttle]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_shuttle_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using 10 fold-cv evaluations with default hyperparameters. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_default_predictor_per_dataset}
\end{figure}


\begin{figure}[h]
\ContinuedFloat 
  \centering 
    \subfloat[waveform]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_waveform_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using 10 fold-cv evaluations with default hyperparameters. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_default_predictor_per_dataset}
\end{figure}


\begin{figure}[h]
\ContinuedFloat 
  \centering 
    \subfloat[winequality]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_winequality_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using 10 fold-cv evaluations with default hyperparameters. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_default_predictor_per_dataset}
\end{figure}


\begin{figure}[h]
\ContinuedFloat 
  \centering 
    \subfloat[yeast]{%
        \includegraphics[width=0.99\linewidth]{images/heatmap/automl_heatmap_yeast_color_flatten.pdf}
      }%
    \caption{Clusters of predictors based on Welch's t-test of each pair of predictors for each dataset using 10 fold-cv evaluations with default hyperparameters. Two predictors that are not statistically different, statistically different and not enough data for statistical testing have a value of 1, 0 and -1, respectively.}
    \label{fig:heatmap_default_predictor_per_dataset}
\end{figure}
 

==> sections/stem_charts.tex <==
\begin{figure}[ht!] 
    \subfloat[abalone\label{fig:stem_chart_abalone}]{%
        \includegraphics[height=1.25\linewidth]{images/stem_charts/stem_chart_abalone.pdf}
        }%
    \hfill
    \subfloat[adult\label{fig:stem_chart_adult}]{%
        \includegraphics[height=1.25\linewidth]{images/stem_charts/stem_chart_adult.pdf}
        }%   
   \caption  Visualisation of the top performing reduction methods (coloured in blue) , the best reduction methods among landmarking, oracle, global leaderboard strategies, the best predictors and their performance in automl-meta and default-meta.
    \label{fig:stem_charts_all_datasets}
\end{figure}        
        
        
        
        
 \begin{figure}[ht!]\ContinuedFloat        
    \subfloat[amazon\label{fig:stem_chart_amazon}]{%
        \includegraphics[height=1.25\linewidth]{images/stem_charts/stem_chart_amazon.pdf}
        }%  
    \hfill
    \subfloat[car\label{fig:stem_chart_car}]{%
        \includegraphics[height=1.25\linewidth]{images/stem_charts/stem_chart_car.pdf}
        }%    
    \caption Visualisation of the top performing reduction methods (coloured in blue) , the best reduction methods among landmarking, oracle, global leaderboard strategies, the best predictors and their performance in automl-meta and default-meta.
    \label{fig:stem_charts_all_datasets}
\end{figure}      
    
    
    
    
\begin{figure}[ht!]\ContinuedFloat     
    \subfloat[cifar10small\label{fig:stem_chart_cifar10small}]{%
        \includegraphics[height=1.25\linewidth]{images/stem_charts/stem_chart_cifar10small.pdf}
        }%
    \hfill
    \subfloat[convex\label{fig:stem_chart_convex}]{%
        \includegraphics[height=1.25\linewidth]{images/stem_charts/stem_chart_convex.pdf}
        }%    
     \caption Visualisation of the top performing reduction methods (coloured in blue) , the best reduction methods among landmarking, oracle, global leaderboard strategies, the best predictors and their performance in automl-meta and default-meta.
    \label{fig:stem_charts_all_datasets}
\end{figure}             
        
        
        
 \begin{figure}[ht!]\ContinuedFloat        
    \hfill
    \subfloat[dexter\label{fig:stem_chart_dexter}]{%
        \includegraphics[height=1.25\linewidth]{images/stem_charts/stem_chart_dexter.pdf}
        }%  
    \hfill
    \subfloat[dorothea\label{fig:stem_chart_dorothea}]{%
        \includegraphics[height=1.25\linewidth]{images/stem_charts/stem_chart_dorothea.pdf}
        }%     
    \caption Visualisation of the top performing reduction methods (coloured in blue) , the best reduction methods among landmarking, oracle, global leaderboard strategies, the best predictors and their performance in automl-meta and default-meta.
    \label{fig:stem_charts_all_datasets}
\end{figure}      

 \begin{figure}[ht!]\ContinuedFloat
    \subfloat[gcredit\label{fig:stem_chart_gcredit}]{%
        \includegraphics[height=1.25\linewidth]{images/stem_charts/stem_chart_gcredit.pdf}
        }%
    \hfill
    \subfloat[gisette\label{fig:stem_chart_gisette}]{%
        \includegraphics[height=1.25\linewidth]{images/stem_charts/stem_chart_gisette.pdf}
        }%    
    \caption Visualisation of the top performing reduction methods (coloured in blue) , the best reduction methods among landmarking, oracle, global leaderboard strategies, the best predictors and their performance in automl-meta and default-meta.
    \label{fig:stem_charts_all_datasets}
\end{figure}              
        
        
 \begin{figure}[ht!]\ContinuedFloat
    \subfloat[kddcup\label{fig:stem_chart_kddcup}]{%
        \includegraphics[height=1.25\linewidth]{images/stem_charts/stem_chart_kddcup.pdf}
        }%  
    \hfill
    \subfloat[krvskp\label{fig:stem_chart_krvskp}]{%
        \includegraphics[height=1.25\linewidth]{images/stem_charts/stem_chart_krvskp.pdf}
        }%
    \caption Visualisation of the top performing reduction methods (coloured in blue) , the best reduction methods among landmarking, oracle, global leaderboard strategies, the best predictors and their performance in automl-meta and default-meta.
    \label{fig:stem_charts_all_datasets}
\end{figure}      


 \begin{figure}[ht!]\ContinuedFloat    
    \subfloat[madelon\label{fig:stem_chart_madelon}]{%
        \includegraphics[height=1.25\linewidth]{images/stem_charts/stem_chart_madelon.pdf}
        }%
    \hfill
    \subfloat[mnist\label{fig:stem_chart_mnist}]{%
        \includegraphics[height=1.25\linewidth]{images/stem_charts/stem_chart_mnist.pdf}
        }%    
    \caption Visualisation of the top performing reduction methods (coloured in blue) , the best reduction methods among landmarking, oracle, global leaderboard strategies, the best predictors and their performance in automl-meta and default-meta.
    \label{fig:stem_charts_all_datasets}
\end{figure}      



 \begin{figure}[ht!]\ContinuedFloat
    \subfloat[secom\label{fig:stem_chart_secom}]{%
        \includegraphics[height=1.25\linewidth]{images/stem_charts/stem_chart_secom.pdf}
        }%  
    \hfill
    \subfloat[semeion\label{fig:stem_chart_semeion}]{%
        \includegraphics[height=1.25\linewidth]{images/stem_charts/stem_chart_semeion.pdf}
        }%
    \caption Visualisation of the top performing reduction methods (coloured in blue) , the best reduction methods among landmarking, oracle, global leaderboard strategies, the best predictors and their performance in automl-meta and default-meta.
    \label{fig:stem_charts_all_datasets}
\end{figure}      



 \begin{figure}[ht!]\ContinuedFloat
    \subfloat[shuttle\label{fig:stem_chart_shuttle}]{%
        \includegraphics[height=1.25\linewidth]{images/stem_charts/stem_chart_shuttle.pdf}
        }%
    \hfill
    \subfloat[waveform\label{fig:stem_chart_waveform}]{%
        \includegraphics[height=1.25\linewidth]{images/stem_charts/stem_chart_waveform.pdf}
        }%    
    \caption Visualisation of the top performing reduction methods (coloured in blue) , the best reduction methods among landmarking, oracle, global leaderboard strategies, the best predictors and their performance in automl-meta and default-meta.
    \label{fig:stem_charts_all_datasets}
\end{figure}      


 \begin{figure}[ht!]\ContinuedFloat
    \subfloat[winequality\label{fig:stem_chart_winequality}]{%
        \includegraphics[height=1.25\linewidth]{images/stem_charts/stem_chart_winequality.pdf}
        }%  
    \hfill
    \subfloat[yeast\label{fig:stem_chart_yeast}]{%
        \includegraphics[height=1.25\linewidth]{images/stem_charts/stem_chart_yeast.pdf}
        }%
   \caption Visualisation of the top performing reduction methods (coloured in blue) , the best reduction methods among landmarking, oracle, global leaderboard strategies, the best predictors and their performance in automl-meta and default-meta.
    \label{fig:stem_charts_all_datasets}
\end{figure}

==> tables/tab_count_common_predictors_best_group.tex <==


\begin{table}[htb!]

\vspace{-0.35cm}

\caption {The number of common predictors between the group of the best predictors of oracle configuration spaces and reduced configuration spaces by strategies (i.e. landmarking and global leaderboard), values of k (i.e., 1, 4, 8, 10, 19) and meta-knowedge  (i.e. \textit{automl-meta} and \textit{default-meta}). Count\_d and count\_e are the number of datasets that have at least one common predictor between the group of the best predictors of oracle configuration spaces and others configuration spaces.
}

\label{tab:count_common_predictors_best_group_strategies_wihout_run_exp}

\centering
\tiny
%\scriptsize
\fontsize{7.5}{7.5}\selectfont
\setlength\tabcolsep{1.5pt}

\begin{tabular}{|ll||llllllllll||llllllllll|}
\hline
\multicolumn{2}{|c|}{\multirow{3}{*}{\textbf{Datasets}}}                                      & \multicolumn{10}{c|}{\textbf{Compare against O1}}                                                                                                                                                                                                                                                                                          & \multicolumn{10}{c|}{\textbf{Compare against O2}}                                                                                                                                                                                                                                                                                          \\ \cline{3-22} 
\multicolumn{2}{|c|}{}                                                                        & \multicolumn{5}{c|}{\textbf{L1}}                                                                                                                                               & \multicolumn{5}{c|}{\textbf{M1}}                                                                                                                          & \multicolumn{5}{c|}{\textbf{L2}}                                                                                                                                               & \multicolumn{5}{c|}{\textbf{M2}}                                                                                                                          \\ \cline{3-22} 
\multicolumn{2}{|c|}{}                                                                        & \multicolumn{1}{l|}{\textbf{k1}} & \multicolumn{1}{l|}{\textbf{k4}} & \multicolumn{1}{l|}{\textbf{k8}} & \multicolumn{1}{l|}{\textbf{k10}} & \multicolumn{1}{l|}{\textbf{k19}} & \multicolumn{1}{l|}{\textbf{k1}} & \multicolumn{1}{l|}{\textbf{k4}} & \multicolumn{1}{l|}{\textbf{k8}} & \multicolumn{1}{l|}{\textbf{k10}} & \textbf{k19} & \multicolumn{1}{l|}{\textbf{k1}} & \multicolumn{1}{l|}{\textbf{k4}} & \multicolumn{1}{l|}{\textbf{k8}} & \multicolumn{1}{l|}{\textbf{k10}} & \multicolumn{1}{l|}{\textbf{k19}} & \multicolumn{1}{l|}{\textbf{k1}} & \multicolumn{1}{l|}{\textbf{k4}} & \multicolumn{1}{l|}{\textbf{k8}} & \multicolumn{1}{l|}{\textbf{k10}} & \textbf{k19} \\ \hline \hline
\multicolumn{1}{|l|}{\multirow{10}{*}{\textbf{'Difficult' datasets}}} & \textbf{car}          & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}            & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}            & 1            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}            & \multicolumn{1}{l|}{0}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}            & 1            \\ \cline{2-22} 
\multicolumn{1}{|l|}{}                                                & \textbf{convex}       & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}            & 1            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}            & \multicolumn{1}{l|}{0}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}            & 1            \\ \cline{2-22} 
\multicolumn{1}{|l|}{}                                                & \textbf{dorothea}     & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{4}           & \multicolumn{1}{l|}{6}            & \multicolumn{1}{l|}{9}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{3}           & \multicolumn{1}{l|}{5}           & \multicolumn{1}{l|}{5}            & 8            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}            & 1            \\ \cline{2-22} 
\multicolumn{1}{|l|}{}                                                & \textbf{gisette}      & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}            & \multicolumn{1}{l|}{0}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}            & 0            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}            & 1            \\ \cline{2-22} 
\multicolumn{1}{|l|}{}                                                & \textbf{mnist}        & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2}            & \multicolumn{1}{l|}{2}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}            & 2            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}            & \multicolumn{1}{l|}{0}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}            & 1            \\ \cline{2-22} 
\multicolumn{1}{|l|}{}                                                & \textbf{amazon}       & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}            & 1            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2}            & \multicolumn{1}{l|}{2}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2}            & 2            \\ \cline{2-22} 
\multicolumn{1}{|l|}{}                                                & \textbf{cifar10small} & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}            & 1            & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{2}            & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2}            & 2            \\ \cline{2-22} 
\multicolumn{1}{|l|}{}                                                & \textbf{madelon}      & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2}            & \multicolumn{1}{l|}{2}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2}            & 2            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{2}            & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2}            & 2            \\ \cline{2-22} 
\multicolumn{1}{|l|}{}                                                & \textbf{winequality}  & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}            & 1            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{2}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}            & 2            \\ \cline{2-22} 
\multicolumn{1}{|l|}{}                                                & \textbf{semeion}      & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}            & 1            & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2}            & \multicolumn{1}{l|}{2}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}            & 3            \\ \hline \hline
\multicolumn{1}{|l|}{\multirow{10}{*}{\textbf{'Easy' datasets}}}      & \textbf{adult}        & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2}            & \multicolumn{1}{l|}{2}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2}            & 2            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2}            & \multicolumn{1}{l|}{4}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2}            & 4            \\ \cline{2-22} 
\multicolumn{1}{|l|}{}                                                & \textbf{krvskp}       & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{2}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2}            & 2            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2}            & \multicolumn{1}{l|}{3}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{3}            & 5            \\ \cline{2-22} 
\multicolumn{1}{|l|}{}                                                & \textbf{waveform}     & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}            & 1            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{4}           & \multicolumn{1}{l|}{4}            & \multicolumn{1}{l|}{5}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2}            & 4            \\ \cline{2-22} 
\multicolumn{1}{|l|}{}                                                & \textbf{shuttle}      & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{2}            & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2}            & 2            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{4}            & \multicolumn{1}{l|}{6}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{4}           & \multicolumn{1}{l|}{5}            & 5            \\ \cline{2-22} 
\multicolumn{1}{|l|}{}                                                & \textbf{dexter}       & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}            & 1            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2}            & \multicolumn{1}{l|}{5}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{3}           & \multicolumn{1}{l|}{3}            & 4            \\ \cline{2-22} 
\multicolumn{1}{|l|}{}                                                & \textbf{kddcup}       & \multicolumn{1}{l|}{-}           & \multicolumn{1}{l|}{-}           & \multicolumn{1}{l|}{-}           & \multicolumn{1}{l|}{-}            & \multicolumn{1}{l|}{-}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{3}            & 7            & \multicolumn{1}{l|}{-}           & \multicolumn{1}{l|}{-}           & \multicolumn{1}{l|}{-}           & \multicolumn{1}{l|}{-}            & \multicolumn{1}{l|}{-}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}            & 3            \\ \cline{2-22} 
\multicolumn{1}{|l|}{}                                                & \textbf{abalone}      & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{2}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2}            & 2            & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{4}           & \multicolumn{1}{l|}{4}            & \multicolumn{1}{l|}{7}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{3}           & \multicolumn{1}{l|}{4}            & 8            \\ \cline{2-22} 
\multicolumn{1}{|l|}{}                                                & \textbf{yeast}        & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2}            & \multicolumn{1}{l|}{3}            & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2}            & 2            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{3}           & \multicolumn{1}{l|}{6}           & \multicolumn{1}{l|}{8}            & \multicolumn{1}{l|}{13}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{4}           & \multicolumn{1}{l|}{5}           & \multicolumn{1}{l|}{7}            & 12           \\ \cline{2-22} 
\multicolumn{1}{|l|}{}                                                & \textbf{gcredit}      & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{1}            & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}            & 1            & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{3}           & \multicolumn{1}{l|}{5}           & \multicolumn{1}{l|}{7}            & \multicolumn{1}{l|}{10}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{4}           & \multicolumn{1}{l|}{7}           & \multicolumn{1}{l|}{9}            & 14           \\ \cline{2-22} 
\multicolumn{1}{|l|}{}                                                & \textbf{secom}        & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{3}           & \multicolumn{1}{l|}{6}           & \multicolumn{1}{l|}{6}            & \multicolumn{1}{l|}{7}            & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{3}            & 6            & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{3}           & \multicolumn{1}{l|}{5}           & \multicolumn{1}{l|}{6}            & \multicolumn{1}{l|}{11}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{4}           & \multicolumn{1}{l|}{5}           & \multicolumn{1}{l|}{6}            & 11           \\ \hline \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{}}                               & \textbf{count\_d}     & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{4}           & \multicolumn{1}{l|}{6}           & \multicolumn{1}{l|}{8}            & \multicolumn{1}{l|}{9}            & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{3}           & \multicolumn{1}{l|}{4}           & \multicolumn{1}{l|}{6}            & 9            & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{7}           & \multicolumn{1}{l|}{7}           & \multicolumn{1}{l|}{7}            & \multicolumn{1}{l|}{7}            & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{4}           & \multicolumn{1}{l|}{6}           & \multicolumn{1}{l|}{6}            & 10           \\ \cline{2-22} 
\multicolumn{1}{|l|}{}                                                & \textbf{count\_e}     & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{4}           & \multicolumn{1}{l|}{7}           & \multicolumn{1}{l|}{9}            & \multicolumn{1}{l|}{9}            & \multicolumn{1}{l|}{3}           & \multicolumn{1}{l|}{6}           & \multicolumn{1}{l|}{9}           & \multicolumn{1}{l|}{9}            & 10           & \multicolumn{1}{l|}{3}           & \multicolumn{1}{l|}{7}           & \multicolumn{1}{l|}{9}           & \multicolumn{1}{l|}{9}            & \multicolumn{1}{l|}{9}            & \multicolumn{1}{l|}{3}           & \multicolumn{1}{l|}{8}           & \multicolumn{1}{l|}{10}          & \multicolumn{1}{l|}{10}           & 10           \\ \hline
\end{tabular}

\end{table}



==> tables/tab_error_20datasets.tex <==


\begin{table*}[htb!]

\vspace{-0.35cm}

\caption {Mean error rate (\%) of the pipelines found by SMAC using different configuration spaces.   }
\label{tab:error_rate_all_methods}

\centering
%\tiny
%\scriptsize
\fontsize{6.0}{8.5}\selectfont
\setlength\tabcolsep{3.0pt}

\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{Dataset}  & \textbf{abalone} & \textbf{adult} & \textbf{amazon} & \textbf{car}  & \textbf{cifar10small} & \textbf{convex} & \textbf{dexter} & \textbf{dorothea} & \textbf{gcredit} & \textbf{gisette} & \textbf{kddcup} & \textbf{krvskp} & \textbf{madelon} & \textbf{mnist} & \textbf{secom} & \textbf{semeion} & \textbf{shuttle} & \textbf{waveform} & \textbf{winequality} & \textbf{yeast} \\ \hline
\textbf{r30}      & 73.81            & 13.22          & \textbf{29.33}  & 0.35          & 66.66                 & 46.72           & 8.21            & 7.21              & 23.26            & \textbf{1.80}    & -               & \textbf{0.38}   & 39.41            & 9.01           & 6.06           & 5.47             & 0.02             & 12.90             & 34.57                & 39.94          \\ \hline
\textbf{baseline} & 73.46            & 13.41          & 58.57           & 2.73          & 75.40                 & 38.99           & 8.81            & 9.30              & 22.83            & 2.93             & \textbf{1.80}   & 0.67            & 26.04            & -              & 6.11           & 8.37             & 0.03             & 12.71             & 37.84                & 39.15          \\ \hline
\textbf{avatar}   & 73.85            & 13.41          & 46.03           & 0.58          & 73.95                 & 30.64           & 8.10            & 6.71              & 22.26            & 2.57             & \textbf{1.80}   & 0.44            & 22.86            & 16.38          & 6.11           & 4.95             & 0.09             & 12.53             & 33.52                & 38.02          \\ \hline
\textbf{L1-k1}    & 72.74            & 12.87          & 74.23           & \textbf{0.33} & 83.42                 & -               & \textbf{5.33}   & -                 & 23.49            & 3.22             & -               & 0.78            & 33.84            & -              & -              & 4.46             & 0.25             & 12.44             & 39.01                & 41.20          \\ \hline
\textbf{L1-k4}    & 72.95            & 14.89          & 31.79           & 0.35          & 70.98                 & 38.79           & 7.19            & -                 & 23.00            & -                & -               & 0.74            & 22.66            & -              & 6.11           & 4.45             & 0.04             & 12.55             & 33.21                & 38.52          \\ \hline
\textbf{L1-k8}    & 73.40            & 14.86          & 38.48           & \textbf{0.33} & 68.15                 & 34.25           & 8.05            & -                 & 23.00            & 6.55             & -               & 0.40            & 22.68            & -              & 6.11           & 4.53             & 0.03             & 12.46             & 33.56                & 37.80          \\ \hline
\textbf{L1-k10}   & 72.98            & 13.99          & 38.48           & \textbf{0.33} & 70.42                 & 25.65           & 7.90            & 6.71              & 22.57            & 6.41             & -               & 0.40            & 22.68            & 2.71           & 6.11           & 4.59             & 0.03             & 12.47             & 33.45                & 37.94          \\ \hline
\textbf{L1-k19}   & 73.27            & 14.16          & 44.06           & 0.38          & -                     & 30.13           & 8.95            & 6.71              & 22.14            & 4.18             & -               & 0.43            & 22.88            & 9.12           & 6.11           & 5.36             & 0.04             & 12.58             & 33.92                & 37.80          \\ \hline
\textbf{L2-k1}    & 74.53            & \textbf{12.86} & 40.23           & \textbf{0.33} & 85.12                 & \textbf{24.11}  & 11.67           & 6.71              & 23.03            & -                & -               & 0.78            & 27.79            & -              & 6.04           & 4.46             & 0.35             & 12.45             & 39.01                & 40.79          \\ \hline
\textbf{L2-k4}    & 74.29            & -              & -               & \textbf{0.33} & 85.68                 & 24.59           & 14.29           & 6.71              & 22.26            & -                & -               & 0.72            & 28.79            & 14.04          & 6.11           & \textbf{4.43}    & 4.41             & 12.42             & 33.12                & 39.23          \\ \hline
\textbf{L2-k8}    & 73.06            & 14.89          & 38.48           & \textbf{0.33} & -                     & 26.43           & -               & 6.96              & 22.46            & -                & -               & 0.47            & 31.39            & 8.24           & 6.06           & 4.46             & 0.02             & 12.57             & 33.32                & 38.98          \\ \hline
\textbf{L2-k10}   & 73.42            & 16.28          & 38.48           & \textbf{0.33} & 70.43                 & 32.91           & 16.79           & 6.92              & 21.97            & -                & -               & 0.51            & 29.31            & -              & 6.09           & 4.48             & 0.02             & 12.53             & 33.46                & 38.89          \\ \hline
\textbf{L2-k19}   & 73.25            & 14.23          & 38.48           & 0.35          & 68.34                 & 37.38           & 7.62            & 7.21              & 22.09            & 4.77             & -               & 0.44            & 24.38            & 14.32          & 6.11           & 5.14             & 0.02             & 12.54             & 33.23                & 37.11          \\ \hline
\textbf{O1-k1}    & 73.77            & -              & -               & 2.60          & -                     & -               & 6.29            & 6.71              & 23.00            & 2.06             & \textbf{1.80}   & 0.55            & 22.66            & 3.96           & 6.11           & 8.65             & 0.02             & 12.57             & \textbf{32.72}       & \textbf{36.65} \\ \hline
\textbf{O1-k4}    & 73.42            & 13.72          & 38.48           & 0.35          & 64.78                 & 26.83           & 5.67            & 6.34              & \textbf{21.23}   & 2.48             & \textbf{1.80}   & 0.41            & 22.72            & -              & 6.11           & 4.77             & 0.02             & 12.50             & 32.91                & 36.90          \\ \hline
\textbf{O1-k8}    & 73.31            & 13.92          & 38.48           & 0.36          & \textbf{57.70}        & 25.51           & 7.80            & 6.34              & 21.49            & 2.43             & \textbf{1.80}   & 0.42            & 23.04            & \textbf{2.68}  & 6.11           & 5.41             & 0.02             & 12.57             & 32.89                & 37.63          \\ \hline
\textbf{O1-k10}   & 73.28            & 13.77          & 38.48           & \textbf{0.33} & 70.72                 & 28.76           & 8.39            & \textbf{5.47}     & 21.91            & 2.36             & -               & 0.44            & 22.91            & 7.42           & 6.11           & 5.52             & 0.02             & 12.54             & 33.29                & 37.42          \\ \hline
\textbf{O1-k19}   & 72.93            & 13.62          & 41.90           & 0.55          & 62.35                 & 31.31           & 8.93            & 7.21              & 21.80            & 2.93             & \textbf{1.80}   & 0.46            & 23.41            & 7.54           & 6.11           & 6.93             & 0.03             & 12.49             & 35.19                & 37.55          \\ \hline
\textbf{O2-k1}    & 73.57            & 13.22          & -               & 0.74          & 89.95                 & -               & 6.29            & -                 & 22.09            & 2.99             & -               & 0.55            & \textbf{20.64}   & 3.63           & 6.11           & 4.46             & 0.02             & 12.46             & \textbf{32.72}       & 40.81          \\ \hline
\textbf{O2-k4}    & 73.58            & 13.80          & 38.48           & 1.07          & -                     & 24.59           & 7.26            & 6.30              & 22.77            & 3.77             & \textbf{1.80}   & 0.40            & 22.66            & 4.45           & 6.11           & 5.16             & 0.02             & 12.48             & 32.88                & 41.10          \\ \hline
\textbf{O2-k8}    & 72.97            & 13.61          & 38.48           & 0.36          & 62.05                 & 28.32           & 7.30            & 6.46              & 22.09            & 2.80             & \textbf{1.80}   & 0.42            & 22.80            & 8.80           & 6.11           & 5.93             & 0.02             & 12.50             & 32.91                & 40.56          \\ \hline
\textbf{O2-k10}   & 73.22            & 13.68          & 38.48           & 0.36          & 100.00                & 30.96           & 7.33            & -                 & 22.03            & 3.60             & \textbf{1.80}   & 0.43            & 22.68            & 3.14           & 6.09           & 6.41             & 0.02             & 12.47             & 33.01                & 39.90          \\ \hline
\textbf{O2-k19}   & 73.32            & 13.93          & -               & 0.35          & 84.29                 & 29.09           & 7.86            & 6.52              & 22.23            & 4.33             & \textbf{1.80}   & 0.46            & 23.59            & 5.46           & 6.11           & 6.66             & 0.03             & 12.59             & 33.56                & 37.55          \\ \hline
\textbf{M1-k1}    & \textbf{72.27}   & 13.85          & 65.43           & 5.92          & 57.77                 & \textbf{24.11}  & 8.45            & 10.08             & 21.74            & 3.35             & \textbf{1.80}   & 0.44            & 26.63            & 4.52           & 6.04           & 5.95             & 0.02             & 13.83             & \textbf{32.72}       & 36.75          \\ \hline
\textbf{M1-k4}    & 72.41            & 13.27          & 61.54           & 2.98          & -                     & 24.89           & 9.95            & -                 & 22.14            & 3.78             & \textbf{1.80}   & 0.40            & 22.64            & 7.54           & \textbf{6.00}  & 6.00             & 0.02             & 13.95             & 32.81                & 36.94          \\ \hline
\textbf{M1-k8}    & 72.89            & 13.82          & -               & 2.71          & 72.34                 & 26.48           & 10.71           & -                 & 22.57            & 4.68             & 1.83            & 0.45            & 22.89            & -              & 6.09           & 7.97             & 0.02             & 12.54             & 33.84                & 37.71          \\ \hline
\textbf{M1-k10}   & 73.26            & 13.70          & 47.68           & 2.93          & 66.15                 & 28.27           & 9.57            & -                 & 22.63            & 5.47             & \textbf{1.80}   & 0.40            & 23.02            & 5.40           & 6.09           & 7.44             & 0.02             & 12.55             & 33.50                & 37.65          \\ \hline
\textbf{M1-k19}   & 73.18            & 14.23          & 38.48           & 0.38          & 70.42                 & 32.21           & 8.76            & -                 & 22.23            & 6.05             & \textbf{1.80}   & 0.48            & 23.78            & 12.93          & 6.11           & 6.01             & 0.02             & 12.57             & 33.39                & 38.00          \\ \hline
\textbf{M2-k1}    & 72.37            & 13.85          & 64.21           & 5.85          & 58.45                 & 24.12           & 8.52            & 7.70              & 22.14            & 3.26             & 2.95            & 0.42            & 24.29            & 4.49           & 6.02           & 5.86             & \textbf{0.02}    & 13.29             & 32.75                & 36.71          \\ \hline
\textbf{M2-k4}    & 72.45            & 13.61          & 55.02           & 5.92          & 61.03                 & 24.25           & 9.10            & -                 & 22.03            & 3.89             & 12.95           & 0.46            & 29.01            & 4.80           & 6.00           & 6.06             & 0.02             & \textbf{12.39}    & 32.96                & 37.09          \\ \hline
\textbf{M2-k8}    & 72.56            & 13.58          & 49.43           & 0.35          & -                     & 25.14           & 8.57            & -                 & 22.20            & 4.14             & \textbf{1.80}   & 0.40            & 27.38            & -              & 6.06           & 4.50             & 0.02             & 12.47             & 33.26                & 37.21          \\ \hline
\textbf{M2-k10}   & 72.73            & 13.79          & 54.57           & 0.36          & 65.56                 & 31.07           & 7.74            & -                 & 22.26            & 2.73             & \textbf{1.80}   & 0.40            & 22.84            & 7.78           & 6.09           & 4.50             & 0.02             & 12.45             & 33.56                & 37.23          \\ \hline
\textbf{M2-k19}   & 72.76            & 13.95          & 53.05           & 0.38          & 66.91                 & 35.94           & 10.95           & -                 & 22.17            & 2.90             & \textbf{1.80}   & 0.46            & 23.21            & -              & 6.11           & 6.15             & 0.02             & 12.49             & 33.31                & 37.75          \\ \hline
\end{tabular}








\end{table*}

==> tables/tab_ranking_correlation.tex <==


\begin{table}[htb!]

\vspace{-0.35cm}

\caption {Correlation coefficients between predictor performance rankings of search space reduction strategies \textit{automl-meta} and \textit{default-meta}.
Strong correlation coefficients are in bold, and weak correlation coefficients are underlined.
}
\label{tab:ranking_correlation_agaist_oracle}

\centering
%\tiny
%\scriptsize
\fontsize{6.5}{6.5}\selectfont
\setlength\tabcolsep{1.5pt}

\begin{tabular}{|l||llllllllll||llllllllll|}
\hline
\multirow{2}{*}{\textbf{Strategies}} & \multicolumn{10}{l|}{\textbf{`Difficult' datasets}}                                                                                                                                                                                                                                                                                                                                         & \multicolumn{10}{l|}{\textbf{`Easy' datasets}}                                                                                                                                                                                                                                                                                                                                   \\ \cline{2-21} 
                                     & \multicolumn{1}{l|}{\textbf{car}}  & \multicolumn{1}{l|}{\textbf{convex}} & \multicolumn{1}{l|}{\textbf{dorothea}} & \multicolumn{1}{l|}{\textbf{gisette}} & \multicolumn{1}{l|}{\textbf{mnist}} & \multicolumn{1}{l|}{\textbf{amazon}} & \multicolumn{1}{l|}{\textbf{cifar10small}} & \multicolumn{1}{l|}{\textbf{madelon}} & \multicolumn{1}{l|}{\textbf{winequality}} & \textbf{semeion} & \multicolumn{1}{l|}{\textbf{adult}} & \multicolumn{1}{l|}{\textbf{krvskp}} & \multicolumn{1}{l|}{\textbf{waveform}} & \multicolumn{1}{l|}{\textbf{shuttle}} & \multicolumn{1}{l|}{\textbf{dexter}} & \multicolumn{1}{l|}{\textbf{kddcup}} & \multicolumn{1}{l|}{\textbf{abalone}} & \multicolumn{1}{l|}{\textbf{yeast}} & \multicolumn{1}{l|}{\textbf{gcredit}} & \textbf{secom} \\ \hline \hline
O1 against O2                        & \multicolumn{1}{l|}{0.55}          & \multicolumn{1}{l|}{0.46}            & \multicolumn{1}{l|}{0.49}              & \multicolumn{1}{l|}{{\ul 0.22}}       & \multicolumn{1}{l|}{0.49}           & \multicolumn{1}{l|}{0.44}            & \multicolumn{1}{l|}{\textbf{0.68}}         & \multicolumn{1}{l|}{{\ul 0.31}}       & \multicolumn{1}{l|}{{\ul 0.33}}           & \textbf{0.79}    & \multicolumn{1}{l|}{0.41}           & \multicolumn{1}{l|}{0.62}            & \multicolumn{1}{l|}{\textbf{0.73}}     & \multicolumn{1}{l|}{0.54}             & \multicolumn{1}{l|}{0.48}            & \multicolumn{1}{l|}{0.43}            & \multicolumn{1}{l|}{0.44}             & \multicolumn{1}{l|}{0.44}           & \multicolumn{1}{l|}{0.46}             & {\ul 0.26}     \\ \hline \hline
L1 against O1                        & \multicolumn{1}{l|}{0.65}          & \multicolumn{1}{l|}{0.54}            & \multicolumn{1}{l|}{0.54}              & \multicolumn{1}{l|}{{\ul 0.08}}       & \multicolumn{1}{l|}{\textbf{0.72}}  & \multicolumn{1}{l|}{\textbf{0.69}}   & \multicolumn{1}{l|}{0.48}                  & \multicolumn{1}{l|}{0.58}             & \multicolumn{1}{l|}{0.64}                 & \textbf{0.72}    & \multicolumn{1}{l|}{0.57}           & \multicolumn{1}{l|}{0.39}            & \multicolumn{1}{l|}{0.53}              & \multicolumn{1}{l|}{0.56}             & \multicolumn{1}{l|}{0.58}            & \multicolumn{1}{l|}{-}               & \multicolumn{1}{l|}{{\ul 0.07}}       & \multicolumn{1}{l|}{\textbf{0.85}}  & \multicolumn{1}{l|}{0.48}             & 0.35           \\ \hline
M1 against O1                        & \multicolumn{1}{l|}{\textbf{0.86}} & \multicolumn{1}{l|}{0.61}            & \multicolumn{1}{l|}{0.53}              & \multicolumn{1}{l|}{0.55}             & \multicolumn{1}{l|}{\textbf{0.76}}  & \multicolumn{1}{l|}{\textbf{0.79}}   & \multicolumn{1}{l|}{0.62}                  & \multicolumn{1}{l|}{\textbf{0.74}}    & \multicolumn{1}{l|}{\textbf{0.78}}        & \textbf{0.71}    & \multicolumn{1}{l|}{\textbf{0.69}}  & \multicolumn{1}{l|}{\textbf{0.74}}   & \multicolumn{1}{l|}{\textbf{0.72}}     & \multicolumn{1}{l|}{\textbf{0.85}}    & \multicolumn{1}{l|}{0.56}            & \multicolumn{1}{l|}{{\ul 0.15}}      & \multicolumn{1}{l|}{\textbf{0.67}}    & \multicolumn{1}{l|}{\textbf{0.91}}  & \multicolumn{1}{l|}{\textbf{0.75}}    & {\ul -   0.01} \\ \hline \hline
L2 against O2                        & \multicolumn{1}{l|}{0.37}          & \multicolumn{1}{l|}{0.53}            & \multicolumn{1}{l|}{0.43}              & \multicolumn{1}{l|}{{\ul -   0.07}}   & \multicolumn{1}{l|}{0.37}           & \multicolumn{1}{l|}{0.44}            & \multicolumn{1}{l|}{{\ul 0.04}}            & \multicolumn{1}{l|}{{\ul 0.29}}       & \multicolumn{1}{l|}{0.53}                 & 0.50             & \multicolumn{1}{l|}{{\ul 0.23}}     & \multicolumn{1}{l|}{{\ul 0.09}}      & \multicolumn{1}{l|}{\textbf{0.78}}     & \multicolumn{1}{l|}{0.38}             & \multicolumn{1}{l|}{{\ul 0.23}}      & \multicolumn{1}{l|}{-}               & \multicolumn{1}{l|}{{\ul 0.29}}       & \multicolumn{1}{l|}{\textbf{0.78}}  & \multicolumn{1}{l|}{{\ul -   0.03}}   & {\ul 0.07}     \\ \hline
M2 against O2                        & \multicolumn{1}{l|}{0.66}          & \multicolumn{1}{l|}{0.49}            & \multicolumn{1}{l|}{{\ul -   0.14}}    & \multicolumn{1}{l|}{0.48}             & \multicolumn{1}{l|}{0.67}           & \multicolumn{1}{l|}{0.53}            & \multicolumn{1}{l|}{0.40}                  & \multicolumn{1}{l|}{0.58}             & \multicolumn{1}{l|}{0.63}                 & 0.58             & \multicolumn{1}{l|}{\textbf{0.67}}  & \multicolumn{1}{l|}{0.62}            & \multicolumn{1}{l|}{\textbf{0.67}}     & \multicolumn{1}{l|}{\textbf{0.73}}    & \multicolumn{1}{l|}{{\ul 0.32}}      & \multicolumn{1}{l|}{-   0.35}        & \multicolumn{1}{l|}{0.58}             & \multicolumn{1}{l|}{\textbf{0.77}}  & \multicolumn{1}{l|}{0.51}             & {\ul -   0.02} \\ \hline
\end{tabular}


\end{table}



==> tables/tab_solution_crash_count.tex <==


\begin{table*}[htb!]

\vspace{-0.35cm}

\caption {T9: Summary table of solution crashes count}
\label{tab:tab_solution_crash_count}

\centering
%\tiny
%\scriptsize
\fontsize{6.0}{8.5}\selectfont
\setlength\tabcolsep{3.0pt}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\rotatebox{90}{\textbf{Dataset}}  & \rotatebox{90}{\textbf{abalone}} & \rotatebox{90}{\textbf{adult}} & \rotatebox{90}{\textbf{amazon}} & \rotatebox{90}{\textbf{car}} & \rotatebox{90}{\textbf{cifar10small}} & \rotatebox{90}{\textbf{convex}} & \rotatebox{90}{\textbf{dexter}}& \rotatebox{90}{\textbf{dorothea}} & \rotatebox{90}{\textbf{gcredit}} & \rotatebox{90}{\textbf{gisette}} & \rotatebox{90}{\textbf{kddcup}} & \rotatebox{90}{\textbf{krvskp}} & \rotatebox{90}{\textbf{madelon}} & \rotatebox{90}{\textbf{mnist}} & \rotatebox{90}{\textbf{secom}} & \rotatebox{90}{\textbf{semeion}} & \rotatebox{90}{\textbf{shuttle}} & \rotatebox{90}{\textbf{waveform}} & \rotatebox{90}{\textbf{winequality}} & \rotatebox{90}{\textbf{yeast}} \\ \hline
\textbf{r30}      & 0                & 0              & 0               & 0            & 2                     & 0               & 1               & 3                 & 0                & 1                & 4               & 0               & 0                & 0              & 0              & 0                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{baseline} & 1                & 2              & 3               & 0            & 3                     & 2               & 4               & 4                 & 0                & 3                & 3               & 0               & 1                & 4              & 1              & 1                & 3                & 2                 & 2                    & 1              \\ \hline
\textbf{avatar}   & 1                & 0              & 2               & 0            & 2                     & 2               & 2               & 3                 & 0                & 3                & 2               & 0               & 0                & 4              & 0              & 0                & 1                & 0                 & 0                    & 0              \\ \hline
\textbf{L1-k1}    & 0                & 0              & 0               & 0            & 3                     & 4               & 0               & 4                 & 0                & 3                & 4               & 0               & 0                & 4              & 4              & 0                & 3                & 0                 & 0                    & 0              \\ \hline
\textbf{L1-k4}    & 0                & 4              & 0               & 0            & 4                     & 4               & 0               & 4                 & 0                & 4                & 4               & 0               & 0                & 4              & 1              & 0                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{L1-k8}    & 0                & 2              & 3               & 0            & 2                     & 2               & 0               & 4                 & 0                & 4                & 4               & 0               & 0                & 4              & 3              & 0                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{L1-k10}   & 0                & 1              & 3               & 0            & 4                     & 2               & 0               & 4                 & 0                & 3                & 4               & 0               & 0                & 4              & 3              & 0                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{L1-k19}   & 0                & 2              & 0               & 0            & 4                     & 0               & 0               & 4                 & 0                & 3                & 4               & 0               & 0                & 4              & 1              & 0                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{L2-k1}    & 0                & 0              & 0               & 0            & 4                     & 0               & 0               & 4                 & 0                & 4                & 4               & 0               & 1                & 4              & 0              & 0                & 3                & 0                 & 0                    & 0              \\ \hline
\textbf{L2-k4}    & 0                & 4              & 4               & 0            & 2                     & 3               & 4               & 4                 & 0                & 4                & 4               & 0               & 0                & 4              & 0              & 0                & 1                & 0                 & 0                    & 0              \\ \hline
\textbf{L2-k8}    & 0                & 2              & 1               & 0            & 4                     & 0               & 4               & 3                 & 0                & 4                & 4               & 0               & 1                & 4              & 0              & 0                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{L2-k10}   & 0                & 3              & 4               & 0            & 3                     & 2               & 3               & 2                 & 0                & 4                & 4               & 0               & 3                & 4              & 1              & 0                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{L2-k19}   & 0                & 1              & 1               & 0            & 4                     & 3               & 2               & 4                 & 0                & 4                & 4               & 0               & 0                & 4              & 0              & 0                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{O1-k1}    & 4                & 4              & 4               & 0            & 4                     & 4               & 0               & 1                 & 0                & 0                & 4               & 0               & 0                & 3              & 0              & 0                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{O1-k4}    & 0                & 4              & 3               & 0            & 3                     & 1               & 0               & 4                 & 0                & 2                & 3               & 0               & 1                & 4              & 0              & 0                & 1                & 0                 & 0                    & 0              \\ \hline
\textbf{O1-k8}    & 0                & 1              & 1               & 0            & 4                     & 2               & 1               & 4                 & 0                & 1                & 3               & 0               & 0                & 4              & 2              & 0                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{O1-k10}   & 0                & 0              & 4               & 0            & 3                     & 1               & 1               & 4                 & 0                & 0                & 4               & 0               & 1                & 4              & 0              & 0                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{O1-k19}   & 0                & 4              & 1               & 0            & 2                     & 0               & 3               & 3                 & 0                & 1                & 2               & 0               & 0                & 4              & 4              & 0                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{O2-k1}    & 2                & 0              & 4               & 0            & 4                     & 4               & 0               & 4                 & 0                & 0                & 4               & 0               & 0                & 4              & 0              & 0                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{O2-k4}    & 0                & 4              & 2               & 0            & 4                     & 2               & 3               & 2                 & 0                & 1                & 4               & 0               & 0                & 4              & 0              & 0                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{O2-k8}    & 2                & 0              & 1               & 0            & 2                     & 1               & 2               & 4                 & 0                & 1                & 2               & 0               & 1                & 4              & 0              & 0                & 0                & 1                 & 0                    & 0              \\ \hline
\textbf{O2-k10}   & 2                & 1              & 2               & 0            & 4                     & 1               & 0               & 4                 & 0                & 0                & 3               & 0               & 0                & 4              & 1              & 1                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{O2-k19}   & 0                & 2              & 4               & 0            & 4                     & 1               & 1               & 3                 & 0                & 2                & 2               & 0               & 2                & 3              & 0              & 0                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{M1-k1}    & 0                & 0              & 0               & 0            & 0                     & 0               & 1               & 0                 & 0                & 0                & 0               & 0               & 0                & 0              & 0              & 0                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{M1-k4}    & 0                & 0              & 0               & 0            & 4                     & 0               & 0               & 4                 & 0                & 0                & 0               & 0               & 0                & 1              & 0              & 0                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{M1-k8}    & 0                & 1              & 4               & 0            & 3                     & 2               & 3               & 4                 & 0                & 3                & 0               & 0               & 0                & 4              & 0              & 0                & 1                & 0                 & 0                    & 0              \\ \hline
\textbf{M1-k10}   & 0                & 1              & 2               & 0            & 3                     & 2               & 0               & 4                 & 0                & 4                & 2               & 0               & 0                & 4              & 0              & 0                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{M1-k19}   & 1                & 1              & 3               & 0            & 4                     & 1               & 0               & 4                 & 0                & 2                & 4               & 0               & 0                & 3              & 3              & 0                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{M2-k1}    & 0                & 0              & 0               & 0            & 0                     & 0               & 0               & 0                 & 0                & 0                & 0               & 0               & 0                & 0              & 0              & 0                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{M2-k4}    & 0                & 0              & 2               & 0            & 1                     & 0               & 0               & 4                 & 0                & 0                & 2               & 0               & 0                & 1              & 0              & 0                & 0                & 1                 & 0                    & 0              \\ \hline
\textbf{M2-k8}    & 0                & 1              & 4               & 0            & 4                     & 2               & 0               & 4                 & 0                & 4                & 1               & 0               & 0                & 4              & 0              & 0                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{M2-k10}   & 0                & 0              & 1               & 0            & 3                     & 1               & 1               & 4                 & 0                & 0                & 1               & 0               & 0                & 1              & 0              & 0                & 0                & 0                 & 0                    & 0              \\ \hline
\textbf{M2-k19}   & 0                & 1              & 3               & 0            & 4                     & 2               & 2               & 4                 & 0                & 4                & 4               & 0               & 0                & 4              & 1              & 0                & 0                & 0                 & 0                    & 0              \\ \hline \hline
\textbf{Average}  & 0.39             & 1.39           & 2.00            & 0.00         & 3.06                  & 1.55            & 1.15            & 3.39              & 0.00             & 2.09             & 2.85            & 0.00            & 0.33             & 3.27           & 0.76           & 0.06             & 0.39             & 0.12              & 0.06                 & 0.03           \\ \hline
\end{tabular}

\end{table*}
